Fundamental Limits of DNA Storage Systems

Due to its longevity and enormous information density, DNA is an attractive medium for archival storage. In this work, we study the fundamental limits and tradeoffs of DNA-based storage systems under a simple model, motivated by current technological constraints on DNA synthesis and sequencing. Our model captures two key distinctive aspects of DNA storage systems: (1) the data is written onto many short DNA molecules that are stored in an unordered way and (2) the data is read by randomly sampling from this DNA pool. Under this model, we characterize the storage capacity, and show that a simple index-based coding scheme is optimal.

==> achievability.tex <==
% !TEX root = DNA_storage_main.tex


Suppose we use the first $\log \M$ bits in each molecule to encode a distinct tag for each molecule.
Then we have $\len - \log \M = \len(1 - 1/\beta)$ symbols per molecule to encode data, and the channel effectively becomes an erasure channel where each symbol (i.e., each molecule) is erased with probability $(1 - 1/\M)^{\M \cNM}$. 
The storage rate $R_s$ achieved is thus $(1-e^{-\cNM})(1-1/\beta)$ (recall that $\lim_{\M\to\infty} (1 - 1/\M)^{\M \cNM} = e^{-\cNM}$). 
%, which agrees with the information theoretic bound in Theorem 1.


%\aln{
%\left( \left| \{ i : \
%}

